State Consensus for Discrete-time Multi-agent Systems over Time-varying Graphs

We study the state consensus problem for linear shift-invariant discrete-time homogeneous multi-agent systems (MASs) over time-varying graphs. A novel approach based on the small gain theorem is proposed to design the consensus control protocols for both neutrally stable and neutrally unstable MASs, assuming the uniformly connected graphs. It is shown that the state consensus can be achieved for neutrally stable MASs under a weak uniform observability condition; for neutrally unstable MASs, the state consensus entails a strong uniform observability condition. Two numerical examples are worked out to illustrate our consensus results.

==> References.tex <==
\begin{thebibliography}{1}
                                 % Insert the full references here.

%\bibitem{Abu-Khalaf, 2005} Abu-Khalaf, M., \& Lewis, F. L. (2005). Nearly optimal control laws for nonlinear systems with saturating actuators using a neural network HJB approach. \textit{Automatica}, 41(5), 779--791.
%1
\bibitem{noot}
A. Nedi$\acute{c}$, A. Olshevsky, A. Ozdaglar and J.N. Tsitsiklis, ``On distributed averaging algorithms and quantization effects,'' {\it IEEE Transactions on Automatic Control}, vol.~54, no.~11, pp.~2506--2517, 2009.

\bibitem{jlm}
A. Jadbabaie and J. Lin and A.S. Morse, ``Coordination of groups of mobile autonomous agents using nearest neighbor rules,'' {\it IEEE Transactions on Automatic Control}, vol.~48, no.~6, pp.~988--1001, 2003.

\bibitem{bt}
B.D.O. Anderson and S. Vongpanitlerd, {\it Network Analysis and Synthesis}, Dover, 2006.

\bibitem{bb}
B. Bollob$\acute{a}$s, {\it Modern Graph Theory}, Springer Science $\&$ Business Media, 2013.

\bibitem{xh}
C. Xiao and D.J. Hill, ``Generalizations and new proof of the discrete-time positive real lemma and bounded real lemma,'' {\it IEEE Transactions on Circuits and Systems I: Fundamental Theory and Applications}, vol.~46, no.~6, pp.~740--743, 1999.

\bibitem{bt}
D.P. Bertsekas and J.N. Tsitsiklis, {\it Parallel and Distributed Computation: Numerical Methods}, Englewood Cliffs, NJ: Prentice Hall, 1989.

\bibitem{gml}
G. Gu and L. Marinovici and F. L. Lewis, ``Consensusability of discrete-time dynamic multiagent systems,'' {\it IEEE Transactions on Automatic Control}, vol.~57, no.~8, pp.~2085--2089, 2012.

\bibitem{gq}
G. Gu and L. Qiu, ``Networked control systems for multi-input plants based on polar logarithmic quantization,'' {\it Systems $\&$ Control Letters}, vol.~69, pp.~16--22, 2014.

\bibitem{llylw}
H. Liang and H. Li and Z. Yu and P. Li and W. Wang, ``Cooperative robust containment control for general discrete-time multi-agent systems with external disturbance,'' {\it IET Control Theory Applications}, vol.~11, no.~12, pp.~1928-1937, 2017.

\bibitem{h2017b}
J. Huang, ``The cooperative output regulation problem of discrete-time linear multi-agent systems by the adaptive distributed observer,'' {\it IEEE Transactions on Automatic Control}, vol.~62, no.~4, pp.~1979--1984, 2017.

\bibitem{yh}
J. Huang, ``Cooperative output regulation of discrete-time linear time-delay multi-agent systems,'' {\it IET Control Theory Applications}, vol.~10, no.~16, pp.~2019--2026, 2016.

\bibitem{h2017}
J. Huang, ``The consensus for discrete-time linear multi-agent systems under directed switching networks,'' {\it IEEE Transactions on Automatic Control}, vol.~62, no.~8, pp.~4086-4092, 2017.

\bibitem{h}
J. Huang, {\it Nonlinear Output Regulation: Theory and Applications}, SIAM Publisher, 2004.

\bibitem{yx}
K. You and L. Xie, ``Network topology and communication data rate for consensusability of discrete-time multi-agent systems,'' {\it IEEE Transactions on Automatic Control}, vol.~56, no.~10, pp.~2262--2275, 2011.

\bibitem{zd}
K. Zhou and J.C. Doyle, {\it Essentials of Robust Control}, Prentice hall Upper Saddle River, NJ, 1998.

\bibitem{xbl}
L. Xiao and S. Boyd and S. Lall, ``A scheme for robust distributed sensor fusion based on average consensus,'' {\it IPSN 2005. Fourth International Symposium on Information Processing in Sensor Networks}, April 2005, vol.~3 ,pp.~63--70.

\bibitem{qgc}
L. Qiu and G. Gu and W. Chen, ``Stabilization of networked multi-input systems with channel resource allocation,'' {\it IEEE Transactions on Automatic Control}, vol.~58, no.~3, pp.~554-568, 2013.

\bibitem{gl2012}
M. Green and D.J.N. Limebeer, {\it Linear Robust Control}, Courier Corporation, 2012.

\bibitem{v}
P. Vaidyanathan, ``The discrete-time bounded-real lemma in digital filterin,'' {\it IEEE Transactions on Circuits and Systems}, vol.~32, no.~9, pp.~918--924, 1985.

\bibitem{hc}
R.A. Horn and C.R. Johnson, {\it Matrix Analysis}, Cambridge University Press, 2012.

\bibitem{rm}
R. Merris, ``A survey of graph Laplacians,'' {\it Linear and Multilinear Algebra}, vol.~39, no.~1-2 ,pp.~19--31, 1995.

\bibitem{osfm}
R. Olfati-Saber and J.A. Fax and R.M. Murray, ``Consensus and cooperation in networked multi-agent systems,'' {\it Proceedings of the IEEE}, vol.~95, no.~1, pp.~215--233, 2007.

\bibitem{saber}
R. Olfati-Saber and R.M. Murray, ``Consensus problems in networks of agents with switching topology and time-delays,'' {\it IEEE Transactions on Automatic Control}, vol.~49, no.~9, pp.~1520--1533, 2004.

\bibitem{osm}
R. Olfati-Saber and R.M. Murray, ``Graph rigidity and distributed formation stabilization of multi-vehicle systems,'' {\it Proceedings of the 41st IEEE Conference on Decision and Control}, Dec 2002, vol.~3 ,pp.~2965--2971.

\bibitem{lxsh}
T.C. Lee, W. Xia, Y. Su and J. Huang, ``New stability results for switched discrete-time systems with application to consensus problemss,'' {\it 2016 IEEE 55th Conference on Decision and Control (CDC)}, Dec 2016, pp.~5508--5514.

\bibitem{gl}
T. Glad and L. Ljung, {\it Control theory}, CRC press, 2000.

\bibitem{nc}
W. Ni and D. Cheng, ``Leader-following consensus of multi-agent systems under fixed and switching topologies,'' {\it Systems $\&$ Control Letters}, vol.~59, no.~3, pp.~209--217, 2010.

%\bibitem{rb2008}
%W. Ren and R.W. Beard, {\it Distributed Consensus in Multi-vehicle Cooperative Control}, Communications and Control Engineering Series, London, U.K.: Springer-Verlag., 2008.

\bibitem{rb}
W. Ren and R.W. Beard, ``Consensus seeking in multiagent systems under dynamically changing interaction topologies,'' {\it IEEE Transactions on Automatic Control}, vol.~50, no.~5, pp.~655--661, 2005.

\bibitem{wzc}
X. Wang and J. Zhu and Z. Cheng, ``Synchronization reachable topology and synchronization of discrete-time linear multi-agent systems,'' {\it IEEE Transactions on Automatic Control}, vol.~60, no.~7, pp.~1927--1932, 2015.


\bibitem{sh2012}
Y. Su and J. Huang, ``Two consensus problems for discrete-time multi-agent systems with switching network topology,'' {\it Automatica}, vol.~48, no.~9, pp.~1988--1997, 2012.


%\bibitem{q}
%Z. Qu, {\it Cooperative Control of Dynamical Systems: Applications to Autonomous Vehicless}, Springer Verlag, London, U.K., 2009.


%\bibitem{hh}
%J. Hu and Y. Hong, ``Leader-following coordination of multi-agent systems with coupling time delays,'' {\it Physica A: Statistical Mechanics and its Applications}, vol.~374, no.~2, pp.~853--863, 2007.



%\bibitem{lfth}
%Z. Li and J. Fang and Y. Tang and T. Huang, ``Consensus of linear discrete-time multi-agent systems: A low-gain distributed impulsive strategy,'' {\it IEEE Transactions on Systems, Man, and Cybernetics: Systems}, vol.~PP, no.~99, pp.~1--2, 2017. DOI: 10.1109/TSMC.2017.2692259.






%\bibitem{pcz}
%A. Ponomarev, Z. Chen and H.T. Zhang, ``Discrete-time predictor feedback for consensus of multi-agent systems with delays,'' {\it IEEE Transactions on Automatic Control}, vol.~PP, no.~99, pp.~1927--1932, 2017. DOI:10.1109/TAC.2017.2722860







%\bibitem{xlf}
%X. Xu and L. Liu and G. Feng, ``Consensus of discrete-time linear multi-agent systems with communication, input and output delays,'' {\it IEEE Transactions on Automatic Control}, vol.~PP, no.~99, pp.~1--2, 2017. DOI: 10.1109/TAC.2017.2720703.

































\end{thebibliography}


